The Flexible Group Spatial Keyword Query

We present a new class of service for location based social networks, called the Flexible Group Spatial Keyword Query, which enables a group of users to collectively find a point of interest (POI) that optimizes an aggregate cost function combining both spatial distances and keyword similarities. In addition, our query service allows users to consider the tradeoffs between obtaining a sub-optimal solution for the entire group and obtaining an optimimized solution but only for a subgroup. We propose algorithms to process three variants of the query: (i) the group nearest neighbor with keywords query, which finds a POI that optimizes the aggregate cost function for the whole group of size n, (ii) the subgroup nearest neighbor with keywords query, which finds the optimal subgroup and a POI that optimizes the aggregate cost function for a given subgroup size m (m <= n), and (iii) the multiple subgroup nearest neighbor with keywords query, which finds optimal subgroups and corresponding POIs for each of the subgroup sizes in the range [m, n]. We design query processing algorithms based on branch-and-bound and best-first paradigms. Finally, we provide theoretical bounds and conduct extensive experiments with two real datasets which verify the effectiveness and efficiency of the proposed algorithms.

==> graphs/flickr/cpu/alpha-gnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,730){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(688,947){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1165){\makebox(0,0)[r]{\strut{}$1500$}}%
      \put(688,1382){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$2500$}}%
      \put(688,1817){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(688,2035){\makebox(0,0)[r]{\strut{}$3500$}}%
      \put(688,2252){\makebox(0,0)[r]{\strut{}$4000$}}%
      \put(688,2470){\makebox(0,0)[r]{\strut{}$4500$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$5000$}}%
      \put(784,352){\makebox(0,0){\strut{}0.1}}%
      \put(1506,352){\makebox(0,0){\strut{}0.3}}%
      \put(2227,352){\makebox(0,0){\strut{}0.5}}%
      \put(2949,352){\makebox(0,0){\strut{}0.7}}%
      \put(4031,352){\makebox(0,0){\strut{}1.0}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2407,112){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}GNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}GNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}GNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}GNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/alpha-gnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/cpu/alpha-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,875){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1237){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(688,1962){\makebox(0,0)[r]{\strut{}$4000$}}%
      \put(688,2325){\makebox(0,0)[r]{\strut{}$5000$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$6000$}}%
      \put(784,352){\makebox(0,0){\strut{}0.1}}%
      \put(1506,352){\makebox(0,0){\strut{}0.3}}%
      \put(2227,352){\makebox(0,0){\strut{}0.5}}%
      \put(2949,352){\makebox(0,0){\strut{}0.7}}%
      \put(4031,352){\makebox(0,0){\strut{}1.0}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2407,112){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/alpha-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/cpu/alpha-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,823){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1133){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(688,1444){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(688,1755){\makebox(0,0)[r]{\strut{}$4000$}}%
      \put(688,2066){\makebox(0,0)[r]{\strut{}$5000$}}%
      \put(688,2376){\makebox(0,0)[r]{\strut{}$6000$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$7000$}}%
      \put(784,352){\makebox(0,0){\strut{}0.1}}%
      \put(1506,352){\makebox(0,0){\strut{}0.3}}%
      \put(2227,352){\makebox(0,0){\strut{}0.5}}%
      \put(2949,352){\makebox(0,0){\strut{}0.7}}%
      \put(4031,352){\makebox(0,0){\strut{}1.0}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2407,112){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/alpha-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/cpu/alpha-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,823){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(688,1133){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1444){\makebox(0,0)[r]{\strut{}$1500$}}%
      \put(688,1755){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(688,2066){\makebox(0,0)[r]{\strut{}$2500$}}%
      \put(688,2376){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$3500$}}%
      \put(784,352){\makebox(0,0){\strut{}0.1}}%
      \put(1506,352){\makebox(0,0){\strut{}0.3}}%
      \put(2227,352){\makebox(0,0){\strut{}0.5}}%
      \put(2949,352){\makebox(0,0){\strut{}0.7}}%
      \put(4031,352){\makebox(0,0){\strut{}1.0}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2407,112){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/alpha-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/cpu/groupsize-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,875){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1237){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(688,1962){\makebox(0,0)[r]{\strut{}$4000$}}%
      \put(688,2325){\makebox(0,0)[r]{\strut{}$5000$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$6000$}}%
      \put(784,352){\makebox(0,0){\strut{}10}}%
      \put(1248,352){\makebox(0,0){\strut{}20}}%
      \put(2176,352){\makebox(0,0){\strut{}40}}%
      \put(3103,352){\makebox(0,0){\strut{}60}}%
      \put(4031,352){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2407,112){\makebox(0,0){\strut{}Group Size}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/groupsize-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/cpu/groupsize-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(784,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(784,784){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(784,1056){\makebox(0,0)[r]{\strut{}$4000$}}%
      \put(784,1328){\makebox(0,0)[r]{\strut{}$6000$}}%
      \put(784,1600){\makebox(0,0)[r]{\strut{}$8000$}}%
      \put(784,1871){\makebox(0,0)[r]{\strut{}$10000$}}%
      \put(784,2143){\makebox(0,0)[r]{\strut{}$12000$}}%
      \put(784,2415){\makebox(0,0)[r]{\strut{}$14000$}}%
      \put(784,2687){\makebox(0,0)[r]{\strut{}$16000$}}%
      \put(880,352){\makebox(0,0){\strut{}10}}%
      \put(1330,352){\makebox(0,0){\strut{}20}}%
      \put(2230,352){\makebox(0,0){\strut{}40}}%
      \put(3131,352){\makebox(0,0){\strut{}60}}%
      \put(4031,352){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2455,112){\makebox(0,0){\strut{}Group Size}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/groupsize-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/cpu/groupsize-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,823){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(688,1133){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1444){\makebox(0,0)[r]{\strut{}$1500$}}%
      \put(688,1755){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(688,2066){\makebox(0,0)[r]{\strut{}$2500$}}%
      \put(688,2376){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$3500$}}%
      \put(784,352){\makebox(0,0){\strut{}10}}%
      \put(1248,352){\makebox(0,0){\strut{}20}}%
      \put(2176,352){\makebox(0,0){\strut{}40}}%
      \put(3103,352){\makebox(0,0){\strut{}60}}%
      \put(4031,352){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2407,112){\makebox(0,0){\strut{}Group Size}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/groupsize-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/cpu/keyword-space-size-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,730){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(688,947){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1165){\makebox(0,0)[r]{\strut{}$1500$}}%
      \put(688,1382){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$2500$}}%
      \put(688,1817){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(688,2035){\makebox(0,0)[r]{\strut{}$3500$}}%
      \put(688,2252){\makebox(0,0)[r]{\strut{}$4000$}}%
      \put(688,2470){\makebox(0,0)[r]{\strut{}$4500$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$5000$}}%
      \put(784,352){\makebox(0,0){\strut{}1}}%
      \put(1596,352){\makebox(0,0){\strut{}2}}%
      \put(2408,352){\makebox(0,0){\strut{}3}}%
      \put(3219,352){\makebox(0,0){\strut{}4}}%
      \put(4031,352){\makebox(0,0){\strut{}5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2407,112){\makebox(0,0){\strut{}Keyword Space Size (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/keyword-space-size-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/cpu/keyword-space-size-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,754){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(688,995){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1237){\makebox(0,0)[r]{\strut{}$1500$}}%
      \put(688,1479){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(688,1720){\makebox(0,0)[r]{\strut{}$2500$}}%
      \put(688,1962){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(688,2204){\makebox(0,0)[r]{\strut{}$3500$}}%
      \put(688,2445){\makebox(0,0)[r]{\strut{}$4000$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$4500$}}%
      \put(784,352){\makebox(0,0){\strut{}1}}%
      \put(1596,352){\makebox(0,0){\strut{}2}}%
      \put(2408,352){\makebox(0,0){\strut{}3}}%
      \put(3219,352){\makebox(0,0){\strut{}4}}%
      \put(4031,352){\makebox(0,0){\strut{}5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2407,112){\makebox(0,0){\strut{}Keyword Space Size (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/keyword-space-size-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/cpu/keyword-space-size-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,875){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(688,1237){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$1500$}}%
      \put(688,1962){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(688,2325){\makebox(0,0)[r]{\strut{}$2500$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(784,352){\makebox(0,0){\strut{}1}}%
      \put(1596,352){\makebox(0,0){\strut{}2}}%
      \put(2408,352){\makebox(0,0){\strut{}3}}%
      \put(3219,352){\makebox(0,0){\strut{}4}}%
      \put(4031,352){\makebox(0,0){\strut{}5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2407,112){\makebox(0,0){\strut{}Keyword Space Size (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/keyword-space-size-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/cpu/number-of-keyword-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,730){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(688,947){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1165){\makebox(0,0)[r]{\strut{}$1500$}}%
      \put(688,1382){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$2500$}}%
      \put(688,1817){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(688,2035){\makebox(0,0)[r]{\strut{}$3500$}}%
      \put(688,2252){\makebox(0,0)[r]{\strut{}$4000$}}%
      \put(688,2470){\makebox(0,0)[r]{\strut{}$4500$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$5000$}}%
      \put(784,352){\makebox(0,0){\strut{}1}}%
      \put(1145,352){\makebox(0,0){\strut{}2}}%
      \put(1866,352){\makebox(0,0){\strut{}4}}%
      \put(3309,352){\makebox(0,0){\strut{}8}}%
      \put(4031,352){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2407,112){\makebox(0,0){\strut{}Number of Keywords}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/number-of-keyword-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/cpu/number-of-keyword-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,754){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(688,995){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1237){\makebox(0,0)[r]{\strut{}$1500$}}%
      \put(688,1479){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(688,1720){\makebox(0,0)[r]{\strut{}$2500$}}%
      \put(688,1962){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(688,2204){\makebox(0,0)[r]{\strut{}$3500$}}%
      \put(688,2445){\makebox(0,0)[r]{\strut{}$4000$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$4500$}}%
      \put(784,352){\makebox(0,0){\strut{}1}}%
      \put(1145,352){\makebox(0,0){\strut{}2}}%
      \put(1866,352){\makebox(0,0){\strut{}4}}%
      \put(3309,352){\makebox(0,0){\strut{}8}}%
      \put(4031,352){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2407,112){\makebox(0,0){\strut{}Number of Keywords}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/number-of-keyword-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/cpu/number-of-keyword-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,875){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(688,1237){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$1500$}}%
      \put(688,1962){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(688,2325){\makebox(0,0)[r]{\strut{}$2500$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(784,352){\makebox(0,0){\strut{}1}}%
      \put(1145,352){\makebox(0,0){\strut{}2}}%
      \put(1866,352){\makebox(0,0){\strut{}4}}%
      \put(3309,352){\makebox(0,0){\strut{}8}}%
      \put(4031,352){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2407,112){\makebox(0,0){\strut{}Number of Keywords}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/number-of-keyword-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/cpu/query-space-area-gnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,784){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(688,1056){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1328){\makebox(0,0)[r]{\strut{}$1500$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(688,1871){\makebox(0,0)[r]{\strut{}$2500$}}%
      \put(688,2143){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(688,2415){\makebox(0,0)[r]{\strut{}$3500$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$4000$}}%
      \put(784,352){\makebox(0,0){\strut{}.001}}%
      \put(1380,352){\makebox(0,0){\strut{}.01}}%
      \put(2043,352){\makebox(0,0){\strut{}.02}}%
      \put(2706,352){\makebox(0,0){\strut{}.03}}%
      \put(3368,352){\makebox(0,0){\strut{}.04}}%
      \put(4031,352){\makebox(0,0){\strut{}.05}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2407,112){\makebox(0,0){\strut{}Query Space Area (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}GNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}GNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}GNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}GNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/query-space-area-gnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/cpu/query-space-area-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,730){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(688,947){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1165){\makebox(0,0)[r]{\strut{}$1500$}}%
      \put(688,1382){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$2500$}}%
      \put(688,1817){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(688,2035){\makebox(0,0)[r]{\strut{}$3500$}}%
      \put(688,2252){\makebox(0,0)[r]{\strut{}$4000$}}%
      \put(688,2470){\makebox(0,0)[r]{\strut{}$4500$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$5000$}}%
      \put(784,352){\makebox(0,0){\strut{}.001}}%
      \put(1380,352){\makebox(0,0){\strut{}.01}}%
      \put(2043,352){\makebox(0,0){\strut{}.02}}%
      \put(2706,352){\makebox(0,0){\strut{}.03}}%
      \put(3368,352){\makebox(0,0){\strut{}.04}}%
      \put(4031,352){\makebox(0,0){\strut{}.05}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2407,112){\makebox(0,0){\strut{}Query Space Area (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/query-space-area-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/cpu/query-space-area-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,754){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(688,995){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1237){\makebox(0,0)[r]{\strut{}$1500$}}%
      \put(688,1479){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(688,1720){\makebox(0,0)[r]{\strut{}$2500$}}%
      \put(688,1962){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(688,2204){\makebox(0,0)[r]{\strut{}$3500$}}%
      \put(688,2445){\makebox(0,0)[r]{\strut{}$4000$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$4500$}}%
      \put(784,352){\makebox(0,0){\strut{}.001}}%
      \put(1380,352){\makebox(0,0){\strut{}.01}}%
      \put(2043,352){\makebox(0,0){\strut{}.02}}%
      \put(2706,352){\makebox(0,0){\strut{}.03}}%
      \put(3368,352){\makebox(0,0){\strut{}.04}}%
      \put(4031,352){\makebox(0,0){\strut{}.05}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2407,112){\makebox(0,0){\strut{}Query Space Area (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/query-space-area-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/cpu/query-space-area-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,875){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(688,1237){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$1500$}}%
      \put(688,1962){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(688,2325){\makebox(0,0)[r]{\strut{}$2500$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(784,352){\makebox(0,0){\strut{}.001}}%
      \put(1380,352){\makebox(0,0){\strut{}.01}}%
      \put(2043,352){\makebox(0,0){\strut{}.02}}%
      \put(2706,352){\makebox(0,0){\strut{}.03}}%
      \put(3368,352){\makebox(0,0){\strut{}.04}}%
      \put(4031,352){\makebox(0,0){\strut{}.05}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2407,112){\makebox(0,0){\strut{}Query Space Area (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/query-space-area-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/cpu/topk-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,875){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1237){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(688,1962){\makebox(0,0)[r]{\strut{}$4000$}}%
      \put(688,2325){\makebox(0,0)[r]{\strut{}$5000$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$6000$}}%
      \put(784,352){\makebox(0,0){\strut{}1}}%
      \put(1380,352){\makebox(0,0){\strut{}10}}%
      \put(2043,352){\makebox(0,0){\strut{}20}}%
      \put(2706,352){\makebox(0,0){\strut{}30}}%
      \put(3368,352){\makebox(0,0){\strut{}40}}%
      \put(4031,352){\makebox(0,0){\strut{}50}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2407,112){\makebox(0,0){\strut{}$k$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/topk-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/cpu/topk-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,730){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(688,947){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1165){\makebox(0,0)[r]{\strut{}$1500$}}%
      \put(688,1382){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$2500$}}%
      \put(688,1817){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(688,2035){\makebox(0,0)[r]{\strut{}$3500$}}%
      \put(688,2252){\makebox(0,0)[r]{\strut{}$4000$}}%
      \put(688,2470){\makebox(0,0)[r]{\strut{}$4500$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$5000$}}%
      \put(784,352){\makebox(0,0){\strut{}1}}%
      \put(1380,352){\makebox(0,0){\strut{}10}}%
      \put(2043,352){\makebox(0,0){\strut{}20}}%
      \put(2706,352){\makebox(0,0){\strut{}30}}%
      \put(3368,352){\makebox(0,0){\strut{}40}}%
      \put(4031,352){\makebox(0,0){\strut{}50}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2407,112){\makebox(0,0){\strut{}$k$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/topk-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/cpu/topk-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,875){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(688,1237){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$1500$}}%
      \put(688,1962){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(688,2325){\makebox(0,0)[r]{\strut{}$2500$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$3000$}}%
      \put(784,352){\makebox(0,0){\strut{}1}}%
      \put(1380,352){\makebox(0,0){\strut{}10}}%
      \put(2043,352){\makebox(0,0){\strut{}20}}%
      \put(2706,352){\makebox(0,0){\strut{}30}}%
      \put(3368,352){\makebox(0,0){\strut{}40}}%
      \put(4031,352){\makebox(0,0){\strut{}50}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2407,112){\makebox(0,0){\strut{}$k$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/cpu/topk-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/alpha-gnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,784){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1056){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(592,1328){\makebox(0,0)[r]{\strut{}$300$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(592,1871){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(592,2143){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(592,2415){\makebox(0,0)[r]{\strut{}$700$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$800$}}%
      \put(688,352){\makebox(0,0){\strut{}0.1}}%
      \put(1431,352){\makebox(0,0){\strut{}0.3}}%
      \put(2174,352){\makebox(0,0){\strut{}0.5}}%
      \put(2917,352){\makebox(0,0){\strut{}0.7}}%
      \put(4031,352){\makebox(0,0){\strut{}1.0}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}GNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}GNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}GNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}GNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/alpha-gnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/alpha-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,875){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(688,1237){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(688,1962){\makebox(0,0)[r]{\strut{}$800$}}%
      \put(688,2325){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$1200$}}%
      \put(784,352){\makebox(0,0){\strut{}0.1}}%
      \put(1506,352){\makebox(0,0){\strut{}0.3}}%
      \put(2227,352){\makebox(0,0){\strut{}0.5}}%
      \put(2949,352){\makebox(0,0){\strut{}0.7}}%
      \put(4031,352){\makebox(0,0){\strut{}1.0}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2407,112){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/alpha-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/alpha-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,754){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(688,995){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(688,1237){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(688,1479){\makebox(0,0)[r]{\strut{}$800$}}%
      \put(688,1720){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1962){\makebox(0,0)[r]{\strut{}$1200$}}%
      \put(688,2204){\makebox(0,0)[r]{\strut{}$1400$}}%
      \put(688,2445){\makebox(0,0)[r]{\strut{}$1600$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$1800$}}%
      \put(784,352){\makebox(0,0){\strut{}0.1}}%
      \put(1506,352){\makebox(0,0){\strut{}0.3}}%
      \put(2227,352){\makebox(0,0){\strut{}0.5}}%
      \put(2949,352){\makebox(0,0){\strut{}0.7}}%
      \put(4031,352){\makebox(0,0){\strut{}1.0}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2407,112){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/alpha-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/alpha-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,784){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1056){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(592,1328){\makebox(0,0)[r]{\strut{}$300$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(592,1871){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(592,2143){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(592,2415){\makebox(0,0)[r]{\strut{}$700$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$800$}}%
      \put(688,352){\makebox(0,0){\strut{}0.1}}%
      \put(1431,352){\makebox(0,0){\strut{}0.3}}%
      \put(2174,352){\makebox(0,0){\strut{}0.5}}%
      \put(2917,352){\makebox(0,0){\strut{}0.7}}%
      \put(4031,352){\makebox(0,0){\strut{}1.0}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/alpha-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/groupsize-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,754){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(688,995){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(688,1237){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(688,1479){\makebox(0,0)[r]{\strut{}$800$}}%
      \put(688,1720){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,1962){\makebox(0,0)[r]{\strut{}$1200$}}%
      \put(688,2204){\makebox(0,0)[r]{\strut{}$1400$}}%
      \put(688,2445){\makebox(0,0)[r]{\strut{}$1600$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$1800$}}%
      \put(784,352){\makebox(0,0){\strut{}10}}%
      \put(1248,352){\makebox(0,0){\strut{}20}}%
      \put(2176,352){\makebox(0,0){\strut{}40}}%
      \put(3103,352){\makebox(0,0){\strut{}60}}%
      \put(4031,352){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2407,112){\makebox(0,0){\strut{}Group Size}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/groupsize-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/groupsize-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(784,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(784,784){\makebox(0,0)[r]{\strut{}$2000$}}%
      \put(784,1056){\makebox(0,0)[r]{\strut{}$4000$}}%
      \put(784,1328){\makebox(0,0)[r]{\strut{}$6000$}}%
      \put(784,1600){\makebox(0,0)[r]{\strut{}$8000$}}%
      \put(784,1871){\makebox(0,0)[r]{\strut{}$10000$}}%
      \put(784,2143){\makebox(0,0)[r]{\strut{}$12000$}}%
      \put(784,2415){\makebox(0,0)[r]{\strut{}$14000$}}%
      \put(784,2687){\makebox(0,0)[r]{\strut{}$16000$}}%
      \put(880,352){\makebox(0,0){\strut{}10}}%
      \put(1330,352){\makebox(0,0){\strut{}20}}%
      \put(2230,352){\makebox(0,0){\strut{}40}}%
      \put(3131,352){\makebox(0,0){\strut{}60}}%
      \put(4031,352){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2455,112){\makebox(0,0){\strut{}Group Size}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/groupsize-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/groupsize-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,730){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(688,947){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(688,1165){\makebox(0,0)[r]{\strut{}$300$}}%
      \put(688,1382){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(688,1817){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(688,2034){\makebox(0,0)[r]{\strut{}$700$}}%
      \put(688,2252){\makebox(0,0)[r]{\strut{}$800$}}%
      \put(688,2470){\makebox(0,0)[r]{\strut{}$900$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(784,352){\makebox(0,0){\strut{}10}}%
      \put(1248,352){\makebox(0,0){\strut{}20}}%
      \put(2176,352){\makebox(0,0){\strut{}40}}%
      \put(3103,352){\makebox(0,0){\strut{}60}}%
      \put(4031,352){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2407,112){\makebox(0,0){\strut{}Group Size}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/groupsize-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/keyword-space-size-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,754){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,995){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$300$}}%
      \put(592,1479){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(592,1720){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(592,2204){\makebox(0,0)[r]{\strut{}$700$}}%
      \put(592,2445){\makebox(0,0)[r]{\strut{}$800$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$900$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1524,352){\makebox(0,0){\strut{}2}}%
      \put(2360,352){\makebox(0,0){\strut{}3}}%
      \put(3195,352){\makebox(0,0){\strut{}4}}%
      \put(4031,352){\makebox(0,0){\strut{}5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Keyword Space Size (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/keyword-space-size-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/keyword-space-size-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,875){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(688,1237){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(688,1962){\makebox(0,0)[r]{\strut{}$800$}}%
      \put(688,2325){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$1200$}}%
      \put(784,352){\makebox(0,0){\strut{}1}}%
      \put(1596,352){\makebox(0,0){\strut{}2}}%
      \put(2408,352){\makebox(0,0){\strut{}3}}%
      \put(3219,352){\makebox(0,0){\strut{}4}}%
      \put(4031,352){\makebox(0,0){\strut{}5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2407,112){\makebox(0,0){\strut{}Keyword Space Size (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/keyword-space-size-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/keyword-space-size-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,823){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1133){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(592,1444){\makebox(0,0)[r]{\strut{}$300$}}%
      \put(592,1755){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(592,2066){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(592,2376){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$700$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1524,352){\makebox(0,0){\strut{}2}}%
      \put(2360,352){\makebox(0,0){\strut{}3}}%
      \put(3195,352){\makebox(0,0){\strut{}4}}%
      \put(4031,352){\makebox(0,0){\strut{}5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Keyword Space Size (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/keyword-space-size-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/number-of-keyword-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,754){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,995){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$300$}}%
      \put(592,1479){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(592,1720){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(592,2204){\makebox(0,0)[r]{\strut{}$700$}}%
      \put(592,2445){\makebox(0,0)[r]{\strut{}$800$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$900$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1059,352){\makebox(0,0){\strut{}2}}%
      \put(1802,352){\makebox(0,0){\strut{}4}}%
      \put(3288,352){\makebox(0,0){\strut{}8}}%
      \put(4031,352){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Number of Keywords}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/number-of-keyword-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/number-of-keyword-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,875){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(688,1237){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(688,1962){\makebox(0,0)[r]{\strut{}$800$}}%
      \put(688,2325){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$1200$}}%
      \put(784,352){\makebox(0,0){\strut{}1}}%
      \put(1145,352){\makebox(0,0){\strut{}2}}%
      \put(1866,352){\makebox(0,0){\strut{}4}}%
      \put(3309,352){\makebox(0,0){\strut{}8}}%
      \put(4031,352){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2407,112){\makebox(0,0){\strut{}Number of Keywords}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/number-of-keyword-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/number-of-keyword-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,823){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1133){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(592,1444){\makebox(0,0)[r]{\strut{}$300$}}%
      \put(592,1755){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(592,2066){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(592,2376){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$700$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1059,352){\makebox(0,0){\strut{}2}}%
      \put(1802,352){\makebox(0,0){\strut{}4}}%
      \put(3288,352){\makebox(0,0){\strut{}8}}%
      \put(4031,352){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Number of Keywords}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/number-of-keyword-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/query-space-area-gnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,823){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1133){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(592,1444){\makebox(0,0)[r]{\strut{}$300$}}%
      \put(592,1755){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(592,2066){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(592,2376){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$700$}}%
      \put(688,352){\makebox(0,0){\strut{}.001}}%
      \put(1302,352){\makebox(0,0){\strut{}.01}}%
      \put(1984,352){\makebox(0,0){\strut{}.02}}%
      \put(2667,352){\makebox(0,0){\strut{}.03}}%
      \put(3349,352){\makebox(0,0){\strut{}.04}}%
      \put(4031,352){\makebox(0,0){\strut{}.05}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Query Space Area (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}GNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}GNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}GNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}GNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/query-space-area-gnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/query-space-area-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,754){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,995){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$300$}}%
      \put(592,1479){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(592,1720){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(592,2204){\makebox(0,0)[r]{\strut{}$700$}}%
      \put(592,2445){\makebox(0,0)[r]{\strut{}$800$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$900$}}%
      \put(688,352){\makebox(0,0){\strut{}.001}}%
      \put(1302,352){\makebox(0,0){\strut{}.01}}%
      \put(1984,352){\makebox(0,0){\strut{}.02}}%
      \put(2667,352){\makebox(0,0){\strut{}.03}}%
      \put(3349,352){\makebox(0,0){\strut{}.04}}%
      \put(4031,352){\makebox(0,0){\strut{}.05}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Query Space Area (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/query-space-area-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/query-space-area-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,875){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(688,1237){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(688,1962){\makebox(0,0)[r]{\strut{}$800$}}%
      \put(688,2325){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$1200$}}%
      \put(784,352){\makebox(0,0){\strut{}.001}}%
      \put(1380,352){\makebox(0,0){\strut{}.01}}%
      \put(2043,352){\makebox(0,0){\strut{}.02}}%
      \put(2706,352){\makebox(0,0){\strut{}.03}}%
      \put(3368,352){\makebox(0,0){\strut{}.04}}%
      \put(4031,352){\makebox(0,0){\strut{}.05}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2407,112){\makebox(0,0){\strut{}Query Space Area (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/query-space-area-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/query-space-area-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,823){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1133){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(592,1444){\makebox(0,0)[r]{\strut{}$300$}}%
      \put(592,1755){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(592,2066){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(592,2376){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$700$}}%
      \put(688,352){\makebox(0,0){\strut{}.001}}%
      \put(1302,352){\makebox(0,0){\strut{}.01}}%
      \put(1984,352){\makebox(0,0){\strut{}.02}}%
      \put(2667,352){\makebox(0,0){\strut{}.03}}%
      \put(3349,352){\makebox(0,0){\strut{}.04}}%
      \put(4031,352){\makebox(0,0){\strut{}.05}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Query Space Area (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/query-space-area-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/topk-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,730){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(688,947){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(688,1165){\makebox(0,0)[r]{\strut{}$300$}}%
      \put(688,1382){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(688,1817){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(688,2034){\makebox(0,0)[r]{\strut{}$700$}}%
      \put(688,2252){\makebox(0,0)[r]{\strut{}$800$}}%
      \put(688,2470){\makebox(0,0)[r]{\strut{}$900$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(784,352){\makebox(0,0){\strut{}1}}%
      \put(1380,352){\makebox(0,0){\strut{}10}}%
      \put(2043,352){\makebox(0,0){\strut{}20}}%
      \put(2706,352){\makebox(0,0){\strut{}30}}%
      \put(3368,352){\makebox(0,0){\strut{}40}}%
      \put(4031,352){\makebox(0,0){\strut{}50}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2407,112){\makebox(0,0){\strut{}$k$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/topk-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/topk-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(688,875){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(688,1237){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(688,1962){\makebox(0,0)[r]{\strut{}$800$}}%
      \put(688,2325){\makebox(0,0)[r]{\strut{}$1000$}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{}$1200$}}%
      \put(784,352){\makebox(0,0){\strut{}1}}%
      \put(1380,352){\makebox(0,0){\strut{}10}}%
      \put(2043,352){\makebox(0,0){\strut{}20}}%
      \put(2706,352){\makebox(0,0){\strut{}30}}%
      \put(3368,352){\makebox(0,0){\strut{}40}}%
      \put(4031,352){\makebox(0,0){\strut{}50}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2407,112){\makebox(0,0){\strut{}$k$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/topk-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/flickr/io/topk-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,823){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1133){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(592,1444){\makebox(0,0)[r]{\strut{}$300$}}%
      \put(592,1755){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(592,2066){\makebox(0,0)[r]{\strut{}$500$}}%
      \put(592,2376){\makebox(0,0)[r]{\strut{}$600$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$700$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1302,352){\makebox(0,0){\strut{}10}}%
      \put(1984,352){\makebox(0,0){\strut{}20}}%
      \put(2667,352){\makebox(0,0){\strut{}30}}%
      \put(3349,352){\makebox(0,0){\strut{}40}}%
      \put(4031,352){\makebox(0,0){\strut{}50}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}$k$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/flickr/io/topk-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/scalability/cpu/dataset-size-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(880,512){\makebox(0,0)[r]{\strut{} 0}}%
      \put(880,875){\makebox(0,0)[r]{\strut{} 2000}}%
      \put(880,1237){\makebox(0,0)[r]{\strut{} 4000}}%
      \put(880,1600){\makebox(0,0)[r]{\strut{} 6000}}%
      \put(880,1962){\makebox(0,0)[r]{\strut{} 8000}}%
      \put(880,2325){\makebox(0,0)[r]{\strut{} 10000}}%
      \put(880,2687){\makebox(0,0)[r]{\strut{} 12000}}%
      \put(976,352){\makebox(0,0){\strut{}1M}}%
      \put(1994,352){\makebox(0,0){\strut{}1.5M}}%
      \put(3013,352){\makebox(0,0){\strut{}2M}}%
      \put(4031,352){\makebox(0,0){\strut{}2.5M}}%
      \large
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2503,112){\makebox(0,0){\strut{}Dataset Size}}%
      \normalsize
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}SGNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}SGNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}SGNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}SGNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/scalability/cpu/dataset-size-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/scalability/cpu/dataset-size-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(880,512){\makebox(0,0)[r]{\strut{} 0}}%
      \put(880,730){\makebox(0,0)[r]{\strut{} 1000}}%
      \put(880,947){\makebox(0,0)[r]{\strut{} 2000}}%
      \put(880,1165){\makebox(0,0)[r]{\strut{} 3000}}%
      \put(880,1382){\makebox(0,0)[r]{\strut{} 4000}}%
      \put(880,1600){\makebox(0,0)[r]{\strut{} 5000}}%
      \put(880,1817){\makebox(0,0)[r]{\strut{} 6000}}%
      \put(880,2035){\makebox(0,0)[r]{\strut{} 7000}}%
      \put(880,2252){\makebox(0,0)[r]{\strut{} 8000}}%
      \put(880,2470){\makebox(0,0)[r]{\strut{} 9000}}%
      \put(880,2687){\makebox(0,0)[r]{\strut{} 10000}}%
      \put(976,352){\makebox(0,0){\strut{}1M}}%
      \put(1994,352){\makebox(0,0){\strut{}1.5M}}%
      \put(3013,352){\makebox(0,0){\strut{}2M}}%
      \put(4031,352){\makebox(0,0){\strut{}2.5M}}%
      \large
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2503,112){\makebox(0,0){\strut{}Dataset Size}}%
      \normalsize
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MSGNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MSGNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MSGNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MSGNNK-BB (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/scalability/cpu/dataset-size-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/scalability/io/dataset-size-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(688,512){\makebox(0,0)[r]{\strut{} 0}}%
      \put(688,784){\makebox(0,0)[r]{\strut{} 100}}%
      \put(688,1056){\makebox(0,0)[r]{\strut{} 200}}%
      \put(688,1328){\makebox(0,0)[r]{\strut{} 300}}%
      \put(688,1600){\makebox(0,0)[r]{\strut{} 400}}%
      \put(688,1871){\makebox(0,0)[r]{\strut{} 500}}%
      \put(688,2143){\makebox(0,0)[r]{\strut{} 600}}%
      \put(688,2415){\makebox(0,0)[r]{\strut{} 700}}%
      \put(688,2687){\makebox(0,0)[r]{\strut{} 800}}%
      \put(784,352){\makebox(0,0){\strut{}1M}}%
      \put(1866,352){\makebox(0,0){\strut{}1.5M}}%
      \put(2949,352){\makebox(0,0){\strut{}2M}}%
      \put(4031,352){\makebox(0,0){\strut{}2.5M}}%
      \large
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2407,112){\makebox(0,0){\strut{}Dataset Size}}%
      \normalsize
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}SGNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}SGNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}SGNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}SGNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/scalability/io/dataset-size-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/scalability/io/dataset-size-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(784,512){\makebox(0,0)[r]{\strut{} 0}}%
      \put(784,875){\makebox(0,0)[r]{\strut{} 200}}%
      \put(784,1237){\makebox(0,0)[r]{\strut{} 400}}%
      \put(784,1600){\makebox(0,0)[r]{\strut{} 600}}%
      \put(784,1962){\makebox(0,0)[r]{\strut{} 800}}%
      \put(784,2325){\makebox(0,0)[r]{\strut{} 1000}}%
      \put(784,2687){\makebox(0,0)[r]{\strut{} 1200}}%
      \put(880,352){\makebox(0,0){\strut{}1M}}%
      \put(1930,352){\makebox(0,0){\strut{}1.5M}}%
      \put(2981,352){\makebox(0,0){\strut{}2M}}%
      \put(4031,352){\makebox(0,0){\strut{}2.5M}}%
      \large
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2455,112){\makebox(0,0){\strut{}Dataset Size}}%
      \normalsize
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MSGNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MSGNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MSGNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MSGNNK-BB (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/scalability/io/dataset-size-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/alpha-gnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,784){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1056){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1328){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1871){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2143){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2415){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(688,352){\makebox(0,0){\strut{}0.1}}%
      \put(1431,352){\makebox(0,0){\strut{}0.3}}%
      \put(2174,352){\makebox(0,0){\strut{}0.5}}%
      \put(2917,352){\makebox(0,0){\strut{}0.7}}%
      \put(4031,352){\makebox(0,0){\strut{}1.0}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}GNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}GNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}GNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}GNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/alpha-gnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/alpha-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,730){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,947){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1165){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1382){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1817){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2035){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2252){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(592,2470){\makebox(0,0)[r]{\strut{}$180$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(688,352){\makebox(0,0){\strut{}0.1}}%
      \put(1431,352){\makebox(0,0){\strut{}0.3}}%
      \put(2174,352){\makebox(0,0){\strut{}0.5}}%
      \put(2917,352){\makebox(0,0){\strut{}0.7}}%
      \put(4031,352){\makebox(0,0){\strut{}1.0}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/alpha-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/alpha-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,754){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,995){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1479){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1720){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2204){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2445){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$180$}}%
      \put(688,352){\makebox(0,0){\strut{}0.1}}%
      \put(1431,352){\makebox(0,0){\strut{}0.3}}%
      \put(2174,352){\makebox(0,0){\strut{}0.5}}%
      \put(2917,352){\makebox(0,0){\strut{}0.7}}%
      \put(4031,352){\makebox(0,0){\strut{}1.0}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/alpha-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/alpha-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,823){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1133){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1444){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1755){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,2066){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2376){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(688,352){\makebox(0,0){\strut{}0.1}}%
      \put(1431,352){\makebox(0,0){\strut{}0.3}}%
      \put(2174,352){\makebox(0,0){\strut{}0.5}}%
      \put(2917,352){\makebox(0,0){\strut{}0.7}}%
      \put(4031,352){\makebox(0,0){\strut{}1.0}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/alpha-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/groupsize-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,947){\makebox(0,0)[r]{\strut{}$50$}}%
      \put(592,1382){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1817){\makebox(0,0)[r]{\strut{}$150$}}%
      \put(592,2252){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$250$}}%
      \put(688,352){\makebox(0,0){\strut{}10}}%
      \put(1166,352){\makebox(0,0){\strut{}20}}%
      \put(2121,352){\makebox(0,0){\strut{}40}}%
      \put(3076,352){\makebox(0,0){\strut{}60}}%
      \put(4031,352){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}Group Size}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/groupsize-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/groupsize-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,754){\makebox(0,0)[r]{\strut{}$50$}}%
      \put(592,995){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$150$}}%
      \put(592,1479){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(592,1720){\makebox(0,0)[r]{\strut{}$250$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$300$}}%
      \put(592,2204){\makebox(0,0)[r]{\strut{}$350$}}%
      \put(592,2445){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$450$}}%
      \put(688,352){\makebox(0,0){\strut{}10}}%
      \put(1166,352){\makebox(0,0){\strut{}20}}%
      \put(2121,352){\makebox(0,0){\strut{}40}}%
      \put(3076,352){\makebox(0,0){\strut{}60}}%
      \put(4031,352){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}Group Size}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/groupsize-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/groupsize-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,730){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,947){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1165){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1382){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1817){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2035){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2252){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(592,2470){\makebox(0,0)[r]{\strut{}$180$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(688,352){\makebox(0,0){\strut{}10}}%
      \put(1166,352){\makebox(0,0){\strut{}20}}%
      \put(2121,352){\makebox(0,0){\strut{}40}}%
      \put(3076,352){\makebox(0,0){\strut{}60}}%
      \put(4031,352){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}Group Size}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/groupsize-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/keyword-space-size-gnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,784){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1056){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1328){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1871){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2143){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2415){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1524,352){\makebox(0,0){\strut{}2}}%
      \put(2360,352){\makebox(0,0){\strut{}3}}%
      \put(3195,352){\makebox(0,0){\strut{}4}}%
      \put(4031,352){\makebox(0,0){\strut{}5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}Keyword Space Size (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}GNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}GNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}GNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}GNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/keyword-space-size-gnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/keyword-space-size-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,754){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,995){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1479){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1720){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2204){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2445){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$180$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1524,352){\makebox(0,0){\strut{}2}}%
      \put(2360,352){\makebox(0,0){\strut{}3}}%
      \put(3195,352){\makebox(0,0){\strut{}4}}%
      \put(4031,352){\makebox(0,0){\strut{}5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}Keyword Space Size (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/keyword-space-size-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/keyword-space-size-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,754){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,995){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1479){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1720){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2204){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2445){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$180$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1524,352){\makebox(0,0){\strut{}2}}%
      \put(2360,352){\makebox(0,0){\strut{}3}}%
      \put(3195,352){\makebox(0,0){\strut{}4}}%
      \put(4031,352){\makebox(0,0){\strut{}5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}Keyword Space Size (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/keyword-space-size-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/keyword-space-size-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,823){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1133){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1444){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1755){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,2066){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2376){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1524,352){\makebox(0,0){\strut{}2}}%
      \put(2360,352){\makebox(0,0){\strut{}3}}%
      \put(3195,352){\makebox(0,0){\strut{}4}}%
      \put(4031,352){\makebox(0,0){\strut{}5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}Keyword Space Size (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/keyword-space-size-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/number-of-keyword-gnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,784){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1056){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1328){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1871){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2143){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2415){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1059,352){\makebox(0,0){\strut{}2}}%
      \put(1802,352){\makebox(0,0){\strut{}4}}%
      \put(3288,352){\makebox(0,0){\strut{}8}}%
      \put(4031,352){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}Number of Keywords}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}GNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}GNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}GNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}GNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/number-of-keyword-gnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/number-of-keyword-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,730){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,947){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1165){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1382){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1817){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2035){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2252){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(592,2470){\makebox(0,0)[r]{\strut{}$180$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1059,352){\makebox(0,0){\strut{}2}}%
      \put(1802,352){\makebox(0,0){\strut{}4}}%
      \put(3288,352){\makebox(0,0){\strut{}8}}%
      \put(4031,352){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}Number of Keywords}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/number-of-keyword-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/number-of-keyword-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,754){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,995){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1479){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1720){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2204){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2445){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$180$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1059,352){\makebox(0,0){\strut{}2}}%
      \put(1802,352){\makebox(0,0){\strut{}4}}%
      \put(3288,352){\makebox(0,0){\strut{}8}}%
      \put(4031,352){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}Number of Keywords}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/number-of-keyword-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/number-of-keyword-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,823){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1133){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1444){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1755){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,2066){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2376){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1059,352){\makebox(0,0){\strut{}2}}%
      \put(1802,352){\makebox(0,0){\strut{}4}}%
      \put(3288,352){\makebox(0,0){\strut{}8}}%
      \put(4031,352){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}Number of Keywords}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/number-of-keyword-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/query-space-area-gnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,784){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1056){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1328){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1871){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2143){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2415){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(688,352){\makebox(0,0){\strut{}.001}}%
      \put(1302,352){\makebox(0,0){\strut{}.01}}%
      \put(1984,352){\makebox(0,0){\strut{}.02}}%
      \put(2667,352){\makebox(0,0){\strut{}.03}}%
      \put(3349,352){\makebox(0,0){\strut{}.04}}%
      \put(4031,352){\makebox(0,0){\strut{}.05}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}Query Space Area (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}GNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}GNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}GNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}GNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/query-space-area-gnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/query-space-area-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,754){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,995){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1479){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1720){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2204){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2445){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$180$}}%
      \put(688,352){\makebox(0,0){\strut{}.001}}%
      \put(1302,352){\makebox(0,0){\strut{}.01}}%
      \put(1984,352){\makebox(0,0){\strut{}.02}}%
      \put(2667,352){\makebox(0,0){\strut{}.03}}%
      \put(3349,352){\makebox(0,0){\strut{}.04}}%
      \put(4031,352){\makebox(0,0){\strut{}.05}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}Query Space Area (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/query-space-area-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/query-space-area-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,754){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,995){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1479){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1720){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2204){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2445){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$180$}}%
      \put(688,352){\makebox(0,0){\strut{}.001}}%
      \put(1302,352){\makebox(0,0){\strut{}.01}}%
      \put(1984,352){\makebox(0,0){\strut{}.02}}%
      \put(2667,352){\makebox(0,0){\strut{}.03}}%
      \put(3349,352){\makebox(0,0){\strut{}.04}}%
      \put(4031,352){\makebox(0,0){\strut{}.05}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}Query Space Area (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/query-space-area-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/query-space-area-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,823){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1133){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1444){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1755){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,2066){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2376){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(688,352){\makebox(0,0){\strut{}.001}}%
      \put(1302,352){\makebox(0,0){\strut{}.01}}%
      \put(1984,352){\makebox(0,0){\strut{}.02}}%
      \put(2667,352){\makebox(0,0){\strut{}.03}}%
      \put(3349,352){\makebox(0,0){\strut{}.04}}%
      \put(4031,352){\makebox(0,0){\strut{}.05}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}Query Space Area (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/query-space-area-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/subgroup-size-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,754){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,995){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1479){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1720){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2204){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2445){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$180$}}%
      \put(688,352){\makebox(0,0){\strut{}40}}%
      \put(1524,352){\makebox(0,0){\strut{}50}}%
      \put(2360,352){\makebox(0,0){\strut{}60}}%
      \put(3195,352){\makebox(0,0){\strut{}70}}%
      \put(4031,352){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}Subgroup Size (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/subgroup-size-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/topk-gnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,754){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,995){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1479){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1720){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2204){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2445){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$180$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1302,352){\makebox(0,0){\strut{}10}}%
      \put(1984,352){\makebox(0,0){\strut{}20}}%
      \put(2667,352){\makebox(0,0){\strut{}30}}%
      \put(3349,352){\makebox(0,0){\strut{}40}}%
      \put(4031,352){\makebox(0,0){\strut{}50}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}$k$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}GNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}GNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}GNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}GNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/topk-gnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/topk-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,730){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,947){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1165){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1382){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1817){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2035){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2252){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(592,2470){\makebox(0,0)[r]{\strut{}$180$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1302,352){\makebox(0,0){\strut{}10}}%
      \put(1984,352){\makebox(0,0){\strut{}20}}%
      \put(2667,352){\makebox(0,0){\strut{}30}}%
      \put(3349,352){\makebox(0,0){\strut{}40}}%
      \put(4031,352){\makebox(0,0){\strut{}50}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}$k$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/topk-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/topk-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,730){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,947){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1165){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1382){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1817){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2035){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2252){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(592,2470){\makebox(0,0)[r]{\strut{}$180$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1302,352){\makebox(0,0){\strut{}10}}%
      \put(1984,352){\makebox(0,0){\strut{}20}}%
      \put(2667,352){\makebox(0,0){\strut{}30}}%
      \put(3349,352){\makebox(0,0){\strut{}40}}%
      \put(4031,352){\makebox(0,0){\strut{}50}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}$k$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/topk-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/cpu/topk-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,823){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1133){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1444){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1755){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,2066){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2376){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1302,352){\makebox(0,0){\strut{}10}}%
      \put(1984,352){\makebox(0,0){\strut{}20}}%
      \put(2667,352){\makebox(0,0){\strut{}30}}%
      \put(3349,352){\makebox(0,0){\strut{}40}}%
      \put(4031,352){\makebox(0,0){\strut{}50}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}running time (ms)}}}%
      \put(2359,112){\makebox(0,0){\strut{}$k$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/cpu/topk-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/alpha-gnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,784){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1056){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1328){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1871){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2143){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2415){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(688,352){\makebox(0,0){\strut{}0.1}}%
      \put(1431,352){\makebox(0,0){\strut{}0.3}}%
      \put(2174,352){\makebox(0,0){\strut{}0.5}}%
      \put(2917,352){\makebox(0,0){\strut{}0.7}}%
      \put(4031,352){\makebox(0,0){\strut{}1.0}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}GNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}GNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}GNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}GNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/alpha-gnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/alpha-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,784){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1056){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1328){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1871){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2143){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2415){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(688,352){\makebox(0,0){\strut{}0.1}}%
      \put(1431,352){\makebox(0,0){\strut{}0.3}}%
      \put(2174,352){\makebox(0,0){\strut{}0.5}}%
      \put(2917,352){\makebox(0,0){\strut{}0.7}}%
      \put(4031,352){\makebox(0,0){\strut{}1.0}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/alpha-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/alpha-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,784){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1056){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1328){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1871){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2143){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2415){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(688,352){\makebox(0,0){\strut{}0.1}}%
      \put(1431,352){\makebox(0,0){\strut{}0.3}}%
      \put(2174,352){\makebox(0,0){\strut{}0.5}}%
      \put(2917,352){\makebox(0,0){\strut{}0.7}}%
      \put(4031,352){\makebox(0,0){\strut{}1.0}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/alpha-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/alpha-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,875){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,2325){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(688,352){\makebox(0,0){\strut{}0.1}}%
      \put(1431,352){\makebox(0,0){\strut{}0.3}}%
      \put(2174,352){\makebox(0,0){\strut{}0.5}}%
      \put(2917,352){\makebox(0,0){\strut{}0.7}}%
      \put(4031,352){\makebox(0,0){\strut{}1.0}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/alpha-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/groupsize-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,754){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,995){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1479){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1720){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2204){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2445){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$180$}}%
      \put(688,352){\makebox(0,0){\strut{}10}}%
      \put(1166,352){\makebox(0,0){\strut{}20}}%
      \put(2121,352){\makebox(0,0){\strut{}40}}%
      \put(3076,352){\makebox(0,0){\strut{}60}}%
      \put(4031,352){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Group Size}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/groupsize-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/groupsize-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,754){\makebox(0,0)[r]{\strut{}$50$}}%
      \put(592,995){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$150$}}%
      \put(592,1479){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(592,1720){\makebox(0,0)[r]{\strut{}$250$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$300$}}%
      \put(592,2204){\makebox(0,0)[r]{\strut{}$350$}}%
      \put(592,2445){\makebox(0,0)[r]{\strut{}$400$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$450$}}%
      \put(688,352){\makebox(0,0){\strut{}10}}%
      \put(1166,352){\makebox(0,0){\strut{}20}}%
      \put(2121,352){\makebox(0,0){\strut{}40}}%
      \put(3076,352){\makebox(0,0){\strut{}60}}%
      \put(4031,352){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Group Size}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/groupsize-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/groupsize-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,875){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,2325){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(688,352){\makebox(0,0){\strut{}10}}%
      \put(1166,352){\makebox(0,0){\strut{}20}}%
      \put(2121,352){\makebox(0,0){\strut{}40}}%
      \put(3076,352){\makebox(0,0){\strut{}60}}%
      \put(4031,352){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Group Size}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/groupsize-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/keyword-space-size-gnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,784){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1056){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1328){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1871){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2143){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2415){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1524,352){\makebox(0,0){\strut{}2}}%
      \put(2360,352){\makebox(0,0){\strut{}3}}%
      \put(3195,352){\makebox(0,0){\strut{}4}}%
      \put(4031,352){\makebox(0,0){\strut{}5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Keyword Space Size (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}GNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}GNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}GNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}GNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/keyword-space-size-gnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/keyword-space-size-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,784){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1056){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1328){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1871){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2143){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2415){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1524,352){\makebox(0,0){\strut{}2}}%
      \put(2360,352){\makebox(0,0){\strut{}3}}%
      \put(3195,352){\makebox(0,0){\strut{}4}}%
      \put(4031,352){\makebox(0,0){\strut{}5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Keyword Space Size (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/keyword-space-size-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/keyword-space-size-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,784){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1056){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1328){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1871){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2143){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2415){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1524,352){\makebox(0,0){\strut{}2}}%
      \put(2360,352){\makebox(0,0){\strut{}3}}%
      \put(3195,352){\makebox(0,0){\strut{}4}}%
      \put(4031,352){\makebox(0,0){\strut{}5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Keyword Space Size (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/keyword-space-size-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/keyword-space-size-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,875){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,2325){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1524,352){\makebox(0,0){\strut{}2}}%
      \put(2360,352){\makebox(0,0){\strut{}3}}%
      \put(3195,352){\makebox(0,0){\strut{}4}}%
      \put(4031,352){\makebox(0,0){\strut{}5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Keyword Space Size (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/keyword-space-size-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/number-of-keyword-gnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,784){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1056){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1328){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1871){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2143){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2415){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1059,352){\makebox(0,0){\strut{}2}}%
      \put(1802,352){\makebox(0,0){\strut{}4}}%
      \put(3288,352){\makebox(0,0){\strut{}8}}%
      \put(4031,352){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Number of Keywords}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}GNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}GNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}GNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}GNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/number-of-keyword-gnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/number-of-keyword-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,784){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1056){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1328){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1871){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2143){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2415){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1059,352){\makebox(0,0){\strut{}2}}%
      \put(1802,352){\makebox(0,0){\strut{}4}}%
      \put(3288,352){\makebox(0,0){\strut{}8}}%
      \put(4031,352){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Number of Keywords}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/number-of-keyword-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/number-of-keyword-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,784){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1056){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1328){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1871){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2143){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2415){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1059,352){\makebox(0,0){\strut{}2}}%
      \put(1802,352){\makebox(0,0){\strut{}4}}%
      \put(3288,352){\makebox(0,0){\strut{}8}}%
      \put(4031,352){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Number of Keywords}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/number-of-keyword-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/number-of-keyword-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,875){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,2325){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1059,352){\makebox(0,0){\strut{}2}}%
      \put(1802,352){\makebox(0,0){\strut{}4}}%
      \put(3288,352){\makebox(0,0){\strut{}8}}%
      \put(4031,352){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Number of Keywords}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/number-of-keyword-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/query-space-area-gnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,784){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1056){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1328){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1871){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2143){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2415){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(688,352){\makebox(0,0){\strut{}.001}}%
      \put(1302,352){\makebox(0,0){\strut{}.01}}%
      \put(1984,352){\makebox(0,0){\strut{}.02}}%
      \put(2667,352){\makebox(0,0){\strut{}.03}}%
      \put(3349,352){\makebox(0,0){\strut{}.04}}%
      \put(4031,352){\makebox(0,0){\strut{}.05}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Query Space Area (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}GNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}GNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}GNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}GNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/query-space-area-gnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/query-space-area-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,784){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1056){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1328){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1871){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2143){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2415){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(688,352){\makebox(0,0){\strut{}.001}}%
      \put(1302,352){\makebox(0,0){\strut{}.01}}%
      \put(1984,352){\makebox(0,0){\strut{}.02}}%
      \put(2667,352){\makebox(0,0){\strut{}.03}}%
      \put(3349,352){\makebox(0,0){\strut{}.04}}%
      \put(4031,352){\makebox(0,0){\strut{}.05}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Query Space Area (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/query-space-area-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/query-space-area-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,784){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1056){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1328){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1871){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2143){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2415){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(688,352){\makebox(0,0){\strut{}.001}}%
      \put(1302,352){\makebox(0,0){\strut{}.01}}%
      \put(1984,352){\makebox(0,0){\strut{}.02}}%
      \put(2667,352){\makebox(0,0){\strut{}.03}}%
      \put(3349,352){\makebox(0,0){\strut{}.04}}%
      \put(4031,352){\makebox(0,0){\strut{}.05}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Query Space Area (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/query-space-area-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/query-space-area-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,875){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,2325){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(688,352){\makebox(0,0){\strut{}.001}}%
      \put(1302,352){\makebox(0,0){\strut{}.01}}%
      \put(1984,352){\makebox(0,0){\strut{}.02}}%
      \put(2667,352){\makebox(0,0){\strut{}.03}}%
      \put(3349,352){\makebox(0,0){\strut{}.04}}%
      \put(4031,352){\makebox(0,0){\strut{}.05}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Query Space Area (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/query-space-area-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/subgroup-size-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,784){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1056){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1328){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1871){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2143){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2415){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(688,352){\makebox(0,0){\strut{}40}}%
      \put(1524,352){\makebox(0,0){\strut{}50}}%
      \put(2360,352){\makebox(0,0){\strut{}60}}%
      \put(3195,352){\makebox(0,0){\strut{}70}}%
      \put(4031,352){\makebox(0,0){\strut{}80}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}Subgroup Size (\%)}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/subgroup-size-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/topk-gnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,754){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,995){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1479){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1720){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2204){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2445){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$180$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1302,352){\makebox(0,0){\strut{}10}}%
      \put(1984,352){\makebox(0,0){\strut{}20}}%
      \put(2667,352){\makebox(0,0){\strut{}30}}%
      \put(3349,352){\makebox(0,0){\strut{}40}}%
      \put(4031,352){\makebox(0,0){\strut{}50}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}$k$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}GNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}GNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}GNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}GNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/topk-gnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/topk-sgnnk.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,730){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,947){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1165){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1382){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1817){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2035){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2252){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(592,2470){\makebox(0,0)[r]{\strut{}$180$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$200$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1302,352){\makebox(0,0){\strut{}10}}%
      \put(1984,352){\makebox(0,0){\strut{}20}}%
      \put(2667,352){\makebox(0,0){\strut{}30}}%
      \put(3349,352){\makebox(0,0){\strut{}40}}%
      \put(4031,352){\makebox(0,0){\strut{}50}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}$k$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}FSNNK-BB (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}FSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}FSNNK-BB (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}FSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/topk-sgnnk}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/topk-sgnnke.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,754){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,995){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1479){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,1720){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(592,2204){\makebox(0,0)[r]{\strut{}$140$}}%
      \put(592,2445){\makebox(0,0)[r]{\strut{}$160$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$180$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1302,352){\makebox(0,0){\strut{}10}}%
      \put(1984,352){\makebox(0,0){\strut{}20}}%
      \put(2667,352){\makebox(0,0){\strut{}30}}%
      \put(3349,352){\makebox(0,0){\strut{}40}}%
      \put(4031,352){\makebox(0,0){\strut{}50}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}$k$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-N (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-N (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/topk-sgnnke}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/yelp/io/topk-sgnnker.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,875){\makebox(0,0)[r]{\strut{}$20$}}%
      \put(592,1237){\makebox(0,0)[r]{\strut{}$40$}}%
      \put(592,1600){\makebox(0,0)[r]{\strut{}$60$}}%
      \put(592,1962){\makebox(0,0)[r]{\strut{}$80$}}%
      \put(592,2325){\makebox(0,0)[r]{\strut{}$100$}}%
      \put(592,2687){\makebox(0,0)[r]{\strut{}$120$}}%
      \put(688,352){\makebox(0,0){\strut{}1}}%
      \put(1302,352){\makebox(0,0){\strut{}10}}%
      \put(1984,352){\makebox(0,0){\strut{}20}}%
      \put(2667,352){\makebox(0,0){\strut{}30}}%
      \put(3349,352){\makebox(0,0){\strut{}40}}%
      \put(4031,352){\makebox(0,0){\strut{}50}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(128,1599){\rotatebox{-270}{\makebox(0,0){\strut{}\# page accesses}}}%
      \put(2359,112){\makebox(0,0){\strut{}$k$}}%
      \csname LTb\endcsname%
      \put(3296,2544){\makebox(0,0)[r]{\strut{}MFSNNK-BF (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2384){\makebox(0,0)[r]{\strut{}MFSNNK-R (SUM)}}%
      \csname LTb\endcsname%
      \put(3296,2224){\makebox(0,0)[r]{\strut{}MFSNNK-BF (MAX)}}%
      \csname LTb\endcsname%
      \put(3296,2064){\makebox(0,0)[r]{\strut{}MFSNNK-R (MAX)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphs/yelp/io/topk-sgnnker}}%
    \gplfronttext
  \end{picture}%
\endgroup

